Adaptive Bayesian Power Spectrum Analysis of Multivariate Nonstationary Time Series

This article introduces a nonparametric approach to multivariate time-varying power spectrum analysis. The procedure adaptively partitions a time series into an unknown number of approximately stationary segments, where some spectral components may remain unchanged across segments, allowing components to evolve differently over time. Local spectra within segments are fit through Whittle likelihood based penalized spline models of modified Cholesky components, which provide flexible nonparametric estimates that preserve positive definite structures of spectral matrices. The approach is formulated in a Bayesian framework, in which the number and location of partitions are random, and relies on reversible jump Markov chain and Hamiltonian Monte Carlo methods that can adapt to the unknown number of segments and parameters. By averaging over the distribution of partitions, the approach can approximate both abrupt and slow-varying changes in spectral matrices. Empirical performance is evaluated in simulation studies and illustrated through analyses of electroencephalography during sleep and of the El Ni\~no-Southern Oscillation.

==> locstatbib <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% a

@article{le1953,
	author={Le Cam, L.},
	year={1953},
	title={On some asymptotic properties of maximum likelihood estimates and related Bayes estimates},
	journal={University of California Publications in Statistics},
	volume={103},
	pages={367-386}
}

@Book{le1990,
	author    = {Le Cam, L. and Yang, G.L.},
	title     = "Asymptotics in Statistics: Some Basic Concepts",
	publisher = "Springer",
	year      =  1990,
	address   = "New York"
}

@article{malik1996,
	author={Malik,M. and Bigger,J. T. and Camm,A. J. and Kleiger,R. E. and Malliani,A. and Moss,A. J. and Schwartz,P. J.},
	year={1996},
	title={Heart rate variability: Standards of measurement, physiological interpretation, and clinical use},
	journal={European Heart Journal},
	volume={17},
	number={3},
	pages={354-381}
}


@article{bruce2017,
	author={Bruce, S. A. and Hall, M. H. and Buysse, D. J. and Krafty, R. T.},
	year={2017},
	title={Conditional adaptive {B}ayesian spectral analysis of nonstationay biomedical time series},
	journal={Biometrics},
	pages={In Press}
}

@article{ombao2006,
	author={Ombao,Hernando and Ho, Moon-ho Ringo},
	year={2006},
	title={Time-dependent frequency domain principal components analysis of multichannel non-stationary signals},
	journal={Computational Statistics \& Data Analysis},
	volume={50},
	number={9},
	pages={2339-2360}
}

@article{bohm2009,
	author={B\"{o}hm,Hilmar and von Sachs,Rainer},
	year={2009},
	title={Shrinkage estimation in the frequency domain of multivariate time series},
	journal={Journal of Multivariate Analysis},
	volume={100},
	number={5},
	pages={913-935}
	
}
@article{fiecas2011,
	author={Fiecas,Mark and Ombao,Hernando},
	year={2011},
	title={The generalized shrinkage estimator
	for the analysis of functional connectivity of brain signals},
	journal={The Annals of Applied Statistics},
	volume={5},
	number={2A},
	pages={1102-1125}
}

@article{fiecas2014,
	author={Fiecas,Mark and von Sachs,Rainer},
	year={2014},
	title={Data-driven shrinkage of the spectral density matrix of a high-dimensional time series},
	journal={Electronic Journal of Statistics},
	volume={8},
	number={2},
	pages={2975-3003}	
}

@article{hall2007,
	author={Hall,Martica and Thayer,Julian F. and Germain,Anne and Moul,Douglas and Vasko,Raymond and Puhl,Matthew and Miewald,Jean and Buysse,Daniel J.},
	year={2007},
	title={Psychological stress is associated with heightened physiological arousal during NREM sleep in primary Insomnia},
	journal={Behavioral Sleep Medicine},
	volume={5},
	number={3},
	pages={178-193}
}

@article{qin2009,
	author={Qin,Li and Guo,Wensheng and Litt,Brain},
	year={2009},
	title={A time-frequency functional model for locally stationary time series data},
	journal={Journal of Computational and Graphical Statistics},
	volume={18},
	number={3},
	pages={675-693}
}

@article{fiecas2016,
	author={Fiecas,Mark and Ombao,Hernando},
	year={2016},
	title={Modeling the evolution of dynamic brain processes during an associative learning experiment},
	journal={Journal of the American Statistical Association},
	volume={111},
	number={516},
	pages={1440-1453}
}
@incollection{neal2011,
	author      = "Radford Neal",
	title       = "MCMC using Hamiltonian dynamics",
	editor      = "Steve Brooks and Andrew Gelman and Galin Jones and Xiao-Li Meng",
	booktitle   = "Handbook of Markov Chain Monte Carlo",
	publisher   = "Chapman \& Hall/CRC Press",
	address     = "Boca Raton, FL",
	year        = 2011,
	pages       = "1385-1399"
}

@article{achermann1998,
	author = "Achermann, P. and Borbely, A.",
	title = "Coherence analysis of the human sleep electroencephalogram",
    year = "1998",
    journal = "Neuroscience",
	volume= "85",
	number= "4",
	pages= "1195-1208"
}

@article{merica1997,
	author = "Merica, H. and Bloris, R.",
	title = "Relationship between the time courses of power in the
	frequency bands of human sleep {EEG}",
	year = "1997",
	journal = "Neurophysiol Clin",
	volume= "27",
	pages= "116-128"
}

@Book{abramowitz1964,
 author    = "Milton {Abramowitz} and Irene A. {Stegun}",
 title     = "Handbook of Mathematical Functions with
              Formulas, Graphs, and Mathematical Tables",
 publisher = "Dover",
 year      =  1964,
 address   = "New York"
}


@article{adak1998,
    author  = "Adak, S.",
    title   = "Time-dependent spectral analysis of non-stationary time series",
    journal = "Journal of the American Statistical Association",
    year    = "1998",
    volume  = "93",
    pages   = "1488-1501"
}

@article{aserinsky1955,
    author  = "Aserinsky, E. and Kleitman, N.",
    title   = "Two types of ocular motility occurring in sleep",
    journal = "Journal of Applied Physiology",
    year    = "1955",
    volume  = "8",
    pages   = "1-10"
}

@article{an2000,
	author = "An, S. and Wang, B",
	title = "Interdecadal change of the structure of the ENSO mode and its impact on the ENSO frequency",
	year = "2000",
	journal = "Journal of Climate",
	volume= "13",
	pages= "2044-2055"
}



@article{aronszajn1950,
    author  = "Aronszajn, N.",
    title   = "Thoery of reproducing kernels",
    journal = "American Mathematical Society Transactions",
    year    = "1950",
    volume  = "68",
    pages   = "337-404"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% b

@book{bhatia1996,
    author  = "Bhatia, Rajendra",
    title   = "Matrix Analysis",
    publisher = "New York: Springer",
    year    = "1997"
}

@article{banno2007,
    author  = "Banno, K. and Kryger, M.H.",
    title   = "Sleep apnea: clinical investigations in humans",
    journal = "Sleep Medicine",
    year    = "2007",
    volume  = "1",
    pages   = "2-11"
}


@article{berkowitz1998,
    author  = "Berkowitz, J. and Diebold, F. X.",
    title   = "Bootstrapping multivariate spectra",
    journal = "Review of Economics and Statistics",
    year    = "1998",
    volume  = "80",
    pages   = "664-666"
}


@book{berlinet2004,
    author  = "Berlinet, A. and Thomas-Agnan, C.",
    title   = "Reproducing Kernel Hilbert Spaces in Probability and Statistics",
    publisher = "Boston: Kluwer",
    year    = "2004"
}

@book{brillinger2001,
    author  = "Brillinger, D. R.",
    title   = "Time Series:  Data Analysis and Theory",
    publisher = "Philadelphia: SIAM",
    year    = "2002"
}

@book{brockwell2006,
    author  = "Brockwell, Peter J. and Davis, Richard A.",
    title   = "Time Series:  Theory and Methods",
    publisher = "New York: Springer",
    year    = "2006"
}

@article{brumback1998,
    author  = "Brumback, B. A. and Rice, J. A.",
    title   = "Smoothing spline models for the analysis of nested and crossed samples of curves",
    journal = "Journal of the American Statistical Association",
    year    = "1998",
    volume  = "93",
    pages   = "961-994"
}




@article{buysse2008,
    author  = "Buysse, D. J. and Germain, A. and Hall, M. L. and Moul, D. E. and Nofzinger, E. A. and Begley, A. and Ehler, C. L. and Thompson, W. and Kupfer, D. J.",
    title   = "EEG spectral analysisi in primary insomnia: NREM period effects and sex differences",
    journal = "Sleep",
    year    = "2008",
    volume  = "31",
    pages   = "1673-1682"
}

@article{brook1998,
	author={Brooks,Stephen P. and Gelman,Andrew},
	year={1998},
	title={General Methods for Monitoring Convergence of Iterative Simulations},
	journal={Journal of Computational and Graphical Statistics},
	volume={7},
	number={4},
	pages={434-455}
}

@article{brooks2000,
	author={Brooks,Stephen P. and Giudici, P.},
	year={2000},
	title={MCMC convergence assessment via two-way ANOVA},
	journal={Journal of Computational and Graphical Statistics},
	volume={9},
	number={4},
	pages={266-285}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% c

@inproceedings{coito2011,
	author={Coito,A. L. and Belo,D. and Paiva,T. and Sanches,J. M.},
	year={2011},
	title={Topographic {EEG} brain mapping before, during and after obstructive sleep apnea episodes},
    booktitle = {2011 IEEE International Symposium on Biomedical Imaging: From Nano to Macro},
	pages={1860-1863},
	isbn={1945-7928}
}

@article{cao2010,
    author  = "Cao, Jiguo and Ramsay, James O.",
    title   = "Linear mixed effects modeling by parameter cascading",
    journal = "Journal of the American Statistical Association",
    year    = "2010",
    volume  = "105",
    pages   = "365-374"
}


@article{chandler2006,
    author  = "Chandler, G. and Polonick, W.",
    title   = "Discrimination of locally stationary time series",
    journal = "Journal of the American Statistical Association",
    year    = "2006",
    volume  = "101",
    pages   = "240-253"
}


@article{chen1980,
    author  = "Chen, Z.-G. and Hannan, E. J.",
    title   = "The distribution of periodogram ordinates",
    journal = "Journal of Time Series Analysis",
    year    = "1980",
    volume  = "1",
    pages   = "73-82"
}


@article{chipman1997,
    author  = "Chipman, Hugh A. and Kolaczyk, Eric D. and McCulloch, Robert E.",
    title   = "Adaptive {B}ayesian wavelet shrinkage",
    journal = "Journal of the American Statistical Association",
    year    = "1997",
    volume  = "92",
    pages   = "1413-1421"
}


@article{cho2014,
    author  = "Cho, Haeran and Fryzlewicz, Piotr",
    title   = "Multiple-change-point detection for high dimensional time series via sparsified binary segmentation",
    journal = "Journal of the Royal Statistical Society, Series B",
    year    = "2014",
    volume  = "77",
    pages   = "475-507"
}

@article{cogburn1974,
    author  = "Cogburn, R. and Davis, H. T.",
    title   = "Periodic splines and spectral estimation",
    journal = "Annals of Statistics",
    year    = "1974",
    volume  = "2",
    pages   = "1108-1126"
}


@article{cox1996,
    author  = "Cox, David D. and O'Sullivan, Finbarr",
    title   = "Penalized likelihood-type estimators for generalized nonparametric regression",
    journal = "Journal of Multivariate Analysis",
    year    = "1996",
    volume  = "56",
    pages   = "185-206"
}

@article{cupidon2008,
    author  = "Cupidon, J. and Eubank, R. and Gilliam, D and Ruymgaart, F.",
    title   = "Some properties of canonical correlations and variates in infinite dimensions",
    journal = "Journal of Multivariate Analysis",
    year    = "2008",
    volume  = "99",
    pages   = "1083-1104"
}

@article{colten2006,
    author  = "Colten, H.R. and Altevogt, B.M.",
    title   = "Sleep disorders and sleep deprivation: an unmet publich health problem",
    publisher = "Institute of Medicine",
    year    = "2008",
	address = "Washington, DC"
		
}

@article{castelloe2002,
	author  = "Castelloe, J.M. and Zimmerman, D.L.",
	title   = "Converge assessment for reversible-jump MCMC samplers",
	journal = "Technical Report, Department of Statistics and Actuarial Science, University of Iowa",
	year    = "2002"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% D

@article{dahlhaus1997,
    author  = "Dahlhaus, R.",
    title   = "Fitting time series models to nonstationary processes",
    journal = "Annals of Statistics",
    year    = "1997",
    volume  = "25",
    pages   = "1-39"
}

@article{dahlhaus2012,
	author="Dahlhaus,R.",
	year="2012",
	title="Locally Stationary Processes",
	journal="Handbook of Statistics",
	volume="30",
	pages="351-413"
}

@article{dahlhaus2000,
    author  = "Dahlhaus, R.",
    title   = "A likelihood approximation for locally stationary process",
    journal = "Annals of Statistics",
    year    = "2000",
    volume  = "28",
    pages   = "1762-1794"
}

@article{davis2006,
    author  = "Davis, R.A. and Lee, T. and Rodriguez-Yam, G.A.",
    title   = "Structural break estimation for nonstationary time series models",
    journal = "Journal of American Statistical Association",
    year    = "2006",
    volume  = "101",
    pages   = "223-239"
}

@book{davison1997,
    author = {Davison, A. C. and Hinkley, D. V.},
    publisher = {Cambridge University Press},
    address = {Cambridge},
    title = {{Bootstrap Methods and Their Application}},
    year = {1997}
}


@book{davis1991,
    author = {Brockwell, P. and Davis, R.},
 	title   = "Time Series:  Theory and Methods",
    publisher = "Springer: New York",
    year    = "1991"
}

@article{dai2004,
    author  = "Dai, Ming and Guo, Wensheng",
    title   = {Multivariate spectral analysis using {Cholesky} decomposition},
    journal = "Biometrika",
    year    = "2004",
    volume  = "91",
    pages   = "629-643"
}

@article{di2009,
    author  = "Di, C.-Z. and Crainiceanu, C. M. and Caffo, B. S. and Punjabi, N. M.",
    title   = "Multilevel functional principal component analysis",
    journal = "Annals of Applied Statistics",
    year    = "2009",
    volume  = "3",
    pages   = "458-488"
}



@article{Dumermuth1983,
	author = "Dumermuth,G. and Lange,B. and Lehmann,D. and Meier,C. A. and Dinkelmann,R. and Molinari,L.",
	year = "1983",
	title = "Spectral Analysis of All-Night Sleep {EEG} in Healthy Adults",
	journal = "European Neurology",
	volume= "22",
	number= "5",
	pages= "322-339"
}


@article{diggle1997,
    author  = "Diggle, Peter J. and Al Wasel, Ibrahim",
    title   = "Spectral analysis of replicated biomedical time series",
    journal = "Applied Statistics",
    year    = "1997",
    volume  = "46",
    pages   = "37-71"
}

@article{dunsmuir1979,
    author  = "Dunsmuir, William Thomson Mulhinch",
    title   = "A central limit theorem for parameter estimation in stationary vector time series and its application to models for a signal observed with noise",
    journal = "Annals of Statistics",
    year    = "1979",
    volume  = "7",
    pages   = "490-506"
}


@article{davies1973,
    author  = "Davies, R. B.",
    title   = "Asymptotic inference in stationary {G}aussian time series",
    journal = "Advances in Applied Probabity",
    year    = "1973",
    volume  = "5",
    pages   = "469-497"
}

@article{deistler1978,
    author  = "Deistler, M. and Dunsmuir, W. and Hannan, E. J.",
    title   = "Vector linear time series models: corrections and extensions",
    journal = "Advances in Applied Probabity",
    year    = "1978",
    volume  = "10",
    pages   = "360-372"
}

@article{dingli2002,
	author = "Dingli,K. and Assimakopoulos,T. and Fietze,I. and Witt,C. and Wraith,P. K. and Douglas,N. J.",
	year="2002",
	title="Electroencephalographic spectral analysis: detection of cortical activity changes in sleep apnoea patients",
	journal="European Respiratory Journal",
	volume=”20“,
	pages=”1246-1253“,
}

@article{duane1987,
author={Duane,Simon and Kennedy,A. D. and Pendleton,Brian J. and Roweth,Duncan},
year={1987},
title={Hybrid Monte Carlo},
journal={Physics Letters B},
volume={195},
number={2},
pages={216-222}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% E

@book{eggermont2009,
    author  = "Eggermont, P. P. B. and LaRiccia, V. N.",
    title   = "Maximum Peanlized Likelihood Estimation.  Volume II: Regression",
    publisher = "New York: Springer",
    year    = "2009"
}

@ARTICLE{eubank2004,
title = {Smoothing spline estimation in varying-coefficient models},
author = {Eubank, R. L. and Huang, Chunfeng and Maldonado,   Maldonado,Y. and Wang, Naisyin and Wang, Suojin and Buchanan, R. J.},
year = {2004},
journal = {Journal Of The Royal Statistical Society Series B},
volume = {66},
number = {3},
pages = {653-667}
}

@ARTICLE{eubank2008,
title = {Canonical correlation for stochastic processes},
author = {Eubank, R. L. and Hsing, Tailen},
year = {2008},
journal = {Stochastic Processes and their Applications},
volume = {118},
pages = {1634-1661}
}

@article{eurotask,
    author  = "Malik, M. and Bigger, J. T. and Camm, A. J. and Kleiger, R. E. and Malliani, A. and Moss, A. J. and Schwartz, P. J.",
    title   = "Heart rate variability - standards of measurement, physiological interpretation, and clinical use",
    journal = "Circulation",
    year    = "1996",
    volume  = "93",
    pages   = "1043-1065"
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% f

@article{fay2001,
    author  = "Fay, G. and Soulier, P",
    title   = "The periodogram of and i.i.d. sequence",
    journal = "Stochastic Processes and their Applications",
    year    = "2001",
    volume  = "92",
    pages =  "315-343"
}

@article{fay2002,
    author  = "Fay, G. and Moulines, Eric and Soulier, P",
    title   = "Nonlinear functionals of the periodogram",
    journal = "Jounal of Time Series Analysis",
    year    = "2002",
    volume  = "23",
    pages =  "523-553"
}


@article{franke1992,
    author  = "Franke, J. and Hardle, W.",
    title   = "ON bootstrapping kernel spectral estimates",
    journal = "Annals of Statistics",
    year    = "1992",
    volume  = "20",
    pages   = "121-145"
}

@article{freyermuth2010,
    author  = "Freyermuth, J.-M. and Ombao, H. and von Sachs, R.",
    title   = "Tree-structured wavelet estimation in a mixed effects model for spectra of replicated time series",
    journal = "Journal of the American Statistical Association",
    year    = "2010",
    volume  = "105",
    pages =  "634-646"
}

@article{fryzlewicz2008,
    author  = "Fryzlewicz, P. and Ombao, H.",
    title   = "Consistent classification of non-stationary time series using stochastic wavelet representations",
    journal = "Journal of the American Statistical Association",
    year    = "2008",
    volume  = "In Press"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% g


@article{gardner2005,
    author  = "Gardner, A. B. and Krieger, A. M. and Vachtsevanos, G. and Litt, B.",
    title   = "One-class novelty detection for seizure analysis from intecranial EEG",
    journal = "Journal of Machine Learning Research",
    year    = "2005",
    volume  = "7",
    pages   = "1025-1044"
}


@article{good1971,
    author  = "Good, I. J. and Gaskins, R. A.",
    title   = "Nonparametric roughness penalties for probability desnities",
    journal = "Biometrika",
    year    = "1971",
    volume  = "58",
    pages   = "255-277"
}

@article{gotze1983,
    author  = "G{\"{o}}tze, F. and  Hipp, C.",
    title   = "Asymptotic expansions for sums of weakly dependent random vectors",
    journal = "Z. Wahrsch. Verw. Gebiete",
    year    = "1983",
    volume  = "64",
    pages   = "211-239"
}

@article{grambsch2004,
    author  = "Grambsch, P. and Young, E. A. and Meller, W. H.",
    title   = "Pulsatile luteinizing hormone disruption in depression",
    journal = "Psychoneuroendocrinology",
    year    = "2004",
    volume  = "29",
    pages   = "825-829"
}

@article{green1995,
    author  = "Green, P.",
    title   = "Reversible jump {M}arkov Chain {M}onte {C}arlo computation and {B}ayesian model determination",
    journal = "Biometrika",
    year    = "1995",
    volume  = "4",
    pages   = "711-732"
}

@book{gu2002,
    author  = "Gu, C.",
    title   = "Smoothing Spline ANOVA Models",
    publisher = "New York: Springer-Verlag",
    year    = "2002"
}

@article{gu1992,
    author  = "Gu, Chong",
    title   = {Cross-validating non-{G}aussian data},
    journal = "Journal of Computational and Graphical Statistics",
    year    = "1992",
    volume  = "1",
    pages   = "169-179"
}

@article{gu1992ss,
    author  = "Gu, Chong",
    title   = {Penalized likelihood regression: a {B}ayesian analysis},
    journal = "Statistica Sinica",
    year    = "1992",
    volume  = "2",
    pages   = "255-264"
}

@article{gu1993,
    author  = "Gu, C. and Wahba, G. ",
    title   = "Semiparametric analysis of variance with tensor product thin plate splines",
    journal = "Journal of the Royal Statistical Society, Series B",
    year    = "1993",
    volume  = "55",
    pages   = "353-368"
}


@article{guo2002,
    author  = "Guo, Wensheng",
    title   = "Functional mixed effects models",
    journal = "Biometrics",
    year    = "2002",
    volume  = "58",
    pages   = "121-128"
}

@article{guo2003,
    author  = "Guo, W. and Dai, M. and Ombao, H. and von Sachs, R. ",
    title   = "Smoothing spline ANOVA for time-dependent spectral analysis",
    journal = "Journal of the American Statistical Association",
    year    = "2003",
    volume  = "98",
    pages   = "643-652"
}

@article{guo2006,
    author  = "Guo, W. and Dai, M.",
    title   = "Multivariate time-dependent spectral analysis using {C}holesky decomposition",
    journal = "Statistica Sinica",
    year    = "2006",
    volume  = "16",
    pages   = "825-845"
}

@article{greeeche2008,
	author={Greneche,J. and Saremi,M. and Erhardt,C. and Hoeft,A. and Eschenlauer,A. and Muzet,A. and Tassi,P.},
	year={2008},
	title={Severity of obstructive sleep apnoea/hypopnoea syndrome and subsequent waking EEG spectral power},
	journal={European Respiratory Journal},
	volume={32},
	number={3},
	pages={705-709},
}

@article{gelman1992,
	author={Gelman,Andrew and Rubin,Donald B.},
	year={1992},
	title={Inference from iterative simulation using multiple sequences},
	journal={Statistical Science},
	volume={7},
	number={4},
	pages={457-472}
	
}

@book{gelman2013,
author={Gelman,Andrew and Carlin, John and Stern, Hal and Dunson, David and Vehtari, Aki and Rubin, Donald},
year={2013},
title={{B}ayesian {D}ata {A}nalysis},
publisher={Chapman \& Hall},
address={Boca Baton, London, New York},
edition={3rd}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% h

@article{hall2004,
    author  = "Hall, M. and Vasko, R. and Buysse, D.J. and Ombao, H. and Chen, Q. and Cashmere, J.D. and Kupfer, D.J. and Thayer, J.F.",
    title   = "Acute stress affects heart rate variability during sleep",
    journal = "Psychosomatic Medicine",
    year    = "2004",
    volume  = "66",
    pages   = "56-62"
}

@article{hall2007,
    author  = "Hall,  M. and Thayer, J.F. and Germain, A. and Moul, D. and Vasko, R. and Puhl, M. and  Miewald, J. and Buysse, D.J.",
    title   = "Psychological stress is associated with heightened physiological arousal during {NREM} sleep in primary insomnia",
    journal = "Behavioral Sleep Medicine",
    year    = "2007",
    volume  = "5",
    pages   = "178-193"
}

@book{hannan1970,
    author  = "Hannan, E. J.",
    title   = "Multiple Time Series",
    publisher = "Wiley",
    address="New York",
    year    = "1970"
}


@article{he2003,
    author  = "He, G. and Muller, H.-G. and Wang, J.-L.",
    title   = "Functional canonical analysis for square itegrable stochastic processes",
    journal = "Journal of Multivariate Analysis",
    year    = "2003",
    volume  = "85",
    pages   = "54-77"
}


@article{he2004,
    author  = "He, G. and Muller, H.-G. and Wang, J.-L.",
    title   = "Methods of cannonical analysis for functional data",
    journal = "Journal of Statistical Planning and Inference",
    year    = "2004",
    volume  = "122",
    pages   = "141-159"
}

@article{hotelling1936,
    author  = "Hotelling, H.",
    title   = "Relations between two sets of variates",
    journal = "Biometrika",
    year    = "1936",
    volume  = "28",
    pages   = "321-377"
}


@article{huang2004,
    author  = "Huang, H.-Y. and Ombao, H. and Stoffer, D.",
    title   = "Discrimination and classification of nonstationary time series using the SLEX model",
    journal = "Journal of the American Statistical Association",
    year    = "2004",
    volume  = "99",
    pages   = "763-774"
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% I
@article{iannaccone2001,
    author  = "Iannaccone, Roberto and Coles, Stuart",
    title   = "Semiparametric models and inference for biomedical time series with extra-variation",
    journal = "Biostatistics",
    year    = "2001",
    volume  = "2",
    pages   = "261-276"
}


@Book{iber2007,
 author    = "Iber, C. and Ancoli-Isreal, S. and Chesson, A. and Quan, S. F.",
 title     = "The {AASM} Manual for the Scoring of Sleep and Associated Events",
 publisher = "American Academy of Sleep Medicine",
 year      =  2007,
 address   = "Westchester, I. L.",
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% j


@article{james2000,
    author  = "James, G. M. and Hastie, T. J. and Sugar, C. A.",
    title   = "Principal component models for sparse functional data",
    journal = "Biometrika",
    year    = "2000",
    volume  = "87",
    pages   = "587-602"
}



@article{janas1995,
    author  = "Janas, Daniel and von Sachs, Rainer",
    title   = "Consistency for non-linear functionals of the periodogram of tapered data",
    journal = "Journal of Time Series Analysis",
    year    = "1995",
    volume  = "16",
    pages   = "585-606"
}

@Book{johnson2002,
author = { Johnson, Richard A. and Wichern, Dean W. },
title = { Applied Multivaraite Statistical Analysis},
publisher = { Upper Saddel River: Prentice Hall},
year = { 2002 }
}

@article{johns1991,
	author  = "Johns, MW",
	title   = "A new method for measuring daytime sleepiness: the {E}pworth sleepiness scale",
	journal = "Sleep",
	year    = "1991",
	volume  = "14",
	pages   = "540"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% k

@article{kimeldorf1971,
    author  = "Kimeldorf, George and Wahba, Grace",
    title   = {Some results on {T}chebycheffian spline functions},
    journal = "Journal of Mathematical Analysis and Applications",
    year    = "1971",
    volume  = "33",
    pages = "82-95"
}




@Book{kadison1997,
author = { Kadison, Richard V., and Ringrose, John R. },
title = { Fundamentals of the theory of operator algebras. Vol. I: Elementary Theory},
publisher = { Providence: Americna Mathematical Society},
year = { 1997 }
}

@article{kirch2015,
    author  = "Kirch, Claudia and Muhsal, Birte and Ombao, Hernando",
    title   = "Detection of changes in multivariate time series with application to {EEG} data",
    journal = "Journal of the American Statistical Association",
    year    = "2015",
    volume  = "110",
    pages   = "1197-1216"
}



@book{kitagawa1996,
    author  = "Kitagawa, G. and Gersch, W.",
    title   = "Smoothness Priors Analysis for Time Series",
    publisher = "Lecture Notes in Statistics (Vol. 116), New York: Springer-Verlag",
    year    = "1996"
}


@article{krafty2008,
    author  = "Krafty, R. T. and Gimotty, P. A. and Holtz, D. and Coukos, G. and Guo, W.",
    title   = "Varying coefficient model with unknown within-subject covariance for analysis of tumor growth curves",
    journal = "Biometrics",
    year    = "2008",
    volume  = "64",
    pages = "1023-1031"
}

@article{krafty2008,
    author  = "Krafty, R. T. and Gimotty, P. A. and Holtz, D. and Coukos, G. and Guo, W.",
    title   = "Varying coefficient model with unknown within-subject covariance for analysis of tumor growth curves",
    journal = "Biometrics",
    year    = "2008",
    volume  = "64",
    pages = "1023-1031"
}

@article{krafty2013,
    author  = "Krafty, R. T. and Collinge, W. O.",
    title   = "Penalized multivariate {W}hittle likelihood for power spectrum estimation",
    journal = "Biometrika",
    year    = "2013",
    volume  = "100",
    pages = "447-458"
}

@article{krafty2016,
    author  = "Krafty, R. T. and Rosen, O. and Stoffer, D. S. and Buysse, D. J. and Hall, M. H.",
    title   = "Conditional spectral analysis of replicated multiple time series with application to nocturnal physiology",
    journal = "Journal of the American Statistical Association",
    year    = "2017",
    pages = "In Press"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% l

@article{laird1982,
    author = {Laird, N. M. and Ware, J. H.},
    journal = {Biometrics},
    pages = {963--974},
    title = {Random-effects models for longitudinal data.},
    volume = {38},
    year = {1982}
}


@article{leurgans1993,
    author  = "Leurgans, S. E. and Moyeed, R. A. and Silverman, B. W.",
    title   = "Canonical correlation analysis when the data are curves",
    journal = "Journal of the Royal Statistical Society, B",
    year    = "1993",
    volume  = "55",
    pages   = "54-77"
}


@article{li2008,
    author  = "Li, Yingxing and Ruppert, David",
    title   = "On the asyptotics of penalized splines",
    journal = "Biometrika",
    year    = "2008",
    volume  = "95",
    pages   = "415-436"
}


@article{lin2004,
    author  = "Lin, X. and Wang, N. and Welsh, A. and Carroll, R. J",
    title   = "Equivalent kernels of smoothing splines in nonparametric regression for clustered data.",
    journal = "Biometrika",
    year    = "2004",
    volume  = "91",
    pages   = "177-193"
}

@article{lin2000,
    author  = "Lin, Y.",
    title   = {Tensor product space {ANOVA} models},
    journal = "Annals of Statistics",
    year    = "2000",
    volume  = "28",
    pages   = "734-755"
}

@article{litt2001,
    author  = "Litt, B. and Esteller, R. and Echuaz, J. and D'Alessandro, M. and Shor, R. and Henry, T. and Pennell, P. and Epstein, C. and Bakay, R. and Dichter, M. and Vachtsevanos, G.",
    title   = "Epileptic seizures may begin hours in advance of clinical onset: a report of five patients",
    journal = "Neuron",
    year    = "2001",
    volume  = "30",
    pages   = "51-64"
}


@article{Lombardi1997,
    author  = "Lombardi, F.",
    title   = "Spectral analysis of heart rate variability",
    journal = "Cardiac Electrophysiology Review",
    year    = "1997",
    volume  = "3",
    pages   = "335-337"
}

@article{liang2007,
	author  = "Liang, F. and Liu, C. and Varroll, R.J.",
	title   = "Stochastic approximation in Monte Carlo computation",
	journal = "Journal of American Statistical Association",
	year    = "2007",
	volume  = "102",
	pages   = "305-320"
}

@article{liang2009,
	author  = "Liang, F.",
	title   = "Improving SAMC using smoothing methods: theory and applications to Bayesian model selection problems",
	journal = "Annals of Statistics",
	year    = "2009",
	volume  = "37",
	pages   = "2626-2654"
}


@article{heureux2013,
	author  = "L'Heureux, M. and Lee, S. and Lyon, B.",
	title   = "Recent multidecadal strengthening of the {W}alker circulation across the tropical {P}acific",
	journal = "Nature Climate Change",
	year    = "2013",
	volume  = "3",
	pages   = "571-576"
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% m n

@article{mustafa2005,
author="Mustafa,M. and Erokwu,N. and Ebose,I. and Strohl,K.",
year= "2005",
title= "Sleep problems and the risk for sleep disorders in an outpatient veteran population",
journal= "Sleep and Breathing",
volume= "9",
number= "2",
pages= "57-63",
}


@book{marshall2011,
    author  = "Marshall, Albert W. and Olkin, Ingram and Arnold, Barry C.",
    title   = "Inequalities:  Theory of Majorization and Its Applications",
    publisher = "New York: Springer",
    year    = "2011"
}

@article {molhave1991,
author = {M{\o}lhave, Lars},
title = {Volatile Organic Compounds, Indoor Air Quality and Health},
journal = {Indoor Air},
volume = {1},
pages = {357-376},
year = {1991}
}

@article{montano2009,
    author = {Montano, N. and Porta, A. and Cogliati, C. and Costantino, G. and Tobaldini, E. and Casali, K. R. and Iellamo, F.},
    journal = {Neuroscience \& Biobehavioral Reviews},
    pages = {71--80},
    title = {Heart rate variability explored in the frequency domain: A tool to investigate the link between heart and behavior},
    volume = {33},
    year = {2009}
}


@article{morisson1998,
	author={Morisson,F. and Lavigne,G. and Petit,D. and Nielsen,T. and Malo,J. and Montplaisir,J.},
	year={1998},
	title={Spectral analysis of wakefulness and {REM} sleep {EEG} in patients with sleep apnoea syndrome},
	journal={European Respiratory Journal},
	volume={11},
	number={5},
	pages={1135-1140}
}


@Article{morris2002,
  author={Morris, Jeffrey S.},
  title={{The BLUPs are not ''best'' when it comes to bootstrapping}},
  journal={Statistics \& Probability Letters},
  year=2002,
  volume={56},
  number={4},
  pages={425-430},
  month={February}
}

@article{neal1994,
author={Neal,Radford M.},
year={1994},
title={An Improved Acceptance Procedure for the Hybrid Monte Carlo Algorithm},
journal={Journal of Computational Physics},
volume={111},
number={1},
pages={194-203}
}


@article{neumann1997,
    author  = "Neumann, M. H. and von Sachs, R. ",
    title   = "Wavelet thresholding in anisotropic function classes and application to adaptive estimation of evolutionary spectra",
    journal = "Annals of Statistics",
    year    = "1997",
    volume  = "83",
    pages   = "1134-1143"
}

@article{newey1997,
    author  = "Newey, W. K. ",
    title   = "Convergence rates and asymptotic normality for series estimators",
    journal = "Journal of Econometrics",
    year    = "1997",
    volume  = "79",
    pages   = "147-168"
}

@article{mormann_07,
    author   =  {Mormann, Florian and Andrzejak, Ralph G. and Elger, Christian E. and Lehnertz, Klaus},
    title    =  {Seizure prediction: the long and winding road},
    year     =  {2007},
    journal  =  {Brain},
    volume   =  {130},
    pages    =  {314-333}
}

@article{morris2006,
    author   =  {Morris, J. S. and Carroll, R. J.},
    title    =  {Wavelet-based functional mixed models},
    year     =  {2006},
    journal  =  {Journal of the Royal Statistical Society, Series B},
    volume   =  {68},
    pages    =  {179-199}
}


@article{nychka1996,
AUTHOR = "Nychka, D. and Cummins, D.J.",
TITLE = "Comment on paper by Eilers and Marx",
JOURNAL = "Statistical Science",
VOLUME = "11",
YEAR = "1996",
PAGES = "104-105"
}

@article{nicholls2008,
	AUTHOR = "Nicholls, N.",
	TITLE = "Recent trends in the seasonal and temporal behaviour of the {E}l {N}i\~no--{S}outhern {O}scillation",
	JOURNAL = "Geophysical Research Letters",
	VOLUME = "35",
	YEAR = "2008",
	PAGES = "L19703"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% o

@article{ombao2001,
    author  = "Ombao, H. and Raz, J. and von Sachs, R. and Malow, B. ",
    title   = "Automatic statistical analysis of bivariate nonstationary time series",
    journal = "Journal of the American Statistical Association",
    year    = "2001",
    volume  = "96",
    pages   = "543-560"
}

@article{ombao2002,
    author  = "Ombao, H. and Raz, J. and von Sachs, R. and Guo, W. ",
    title   = "The SLEX model of a non-stationary random process",
    journal = "Annals of the Institute of Statistical Mathematics ",
    year    = "2002",
    volume  = "54",
    pages   = "171-200"
    }

@article{ombao2005,
    author  = "Ombao, H. and von Sachs, R. and Guo, W. ",
    title   = "{SLEX} Analysis of Multivaraite Nonstationary Time Series",
    journal = "Journal of the American Statistical Association",
    year    = "2005",
    volume  = "100",
    pages   = "519-531"
    }




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% P

@article{park2014,
    author  = "Park, Timothy and Eckley, I. A. and Ombao, Hernando C.",
    title   = "Estimating time-evolving partial coherence between signals via multivariate locally stationary wavelet processes",
    journal = "IEEE Transactions on Signal Processing",
    year    = "2014",
    volume  = "62",
    pages   = "5240-5240"
}



@article{pawitan1994,
    author  = "Pawitan, Yudi and O'Sullivan, Finbarr",
    title   = {Nonparametric spectral density estimation using penalized {Whittle} likelihood},
    journal = "Journal of the American Statistical Association",
    year    = "1994",
    volume  = "89",
    pages   = "600-610"
}

@article{pawitan1996,
    author  = "Pawitan, Yudi",
    title   = "Automatic estimation of the cross-spectrum of a bivariate time series",
    journal = "Biometrika",
    year    = "1996",
    volume  = "83",
    pages   = "419-432"
}




@article{priestley1965,
    author  = "Priestley, M. B.",
    title   = "Evolutionary spectral and non-stationary process",
    journal = "Journal of the Royal Statistical Society, Series B",
    year    = "1965",
    volume  = "28",
    pages   = "228-240"
}


@book{priestley1981,
    author  = "Priestley, M. B.",
    title   = "Spectral Analysis and Time Series, Vol. 1 and 2",
    publisher = "London: Academic Press",
    year    = "1981"
}

@article{preuss2015,
    author  = "Preuss, Philip and Puchstein, Ruprecht and Dette, Holger",
    title   = "Detection of multiple structural breaks in multivariate time series",
    journal = "Journal of the American Statistical Association",
    year    = "2015",
    volume  = "110",
    pages   = "654-668"
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% Q
@article{qin2006,
    author  = "Qin, Li and Guo, Wensheng",
    title   = "Functional Mixed-Effects Model for Periodic Data",
    journal = "Biostatistics",
    year    = "2006",
    volume  = "7",
    pages   = "225-234"
}

@article{qin2009,
    author  = "Qin, Li and Litt, Brian and Guo, Wensheng",
    title   = "A Time-frequency Functional Model for Locally Stationary Time Series Data",
    journal = "Journal of Computational and Graphical Statistics",
    year    = "2009",
    volume  = "18",
    pages   = "675-693"
}

@article{qin2009wang,
    author  = "Qin, Li and Wang, Yuedong",
    title   = {{Nonparametric spectral analysis with applications to seizure characterization using EEG time series}},
    journal = "Annals of Applied Statistics",
    year    = "2008",
    volume  = "2",
    pages   = "1432-1451"
}

@article{quiroga2002,
    author  = "Quiroga, R. Q. and Kraskov, A. and Kreuz, T. and Grassberger, P.",
    title   = "Performance of different synchronization measures in real data: {A} case study on electrocenephalographic signals",
    journal = "Phisical Review E",
    year    = "2002",
    volume  = "65",
    pages   = "041903"
}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% R

@article{ramsay1991,
    author  = "Ramsay, J. O. and Danzell, C. J.",
    title   = "Some tools for functional data analysis",
    journal = "Journal of the Royal Statistical Society, B",
    year    = "1991",
    volume  = "53",
    pages   = "539-572"
}



@article{ranpuria2008,
    author  = "Ranpuria, R. and Hall, M. L. and Chan, C. T. and Unruh, M.",
    title   = "Heart rate variability (HRV) in kidney failure: measurement and consequences of reduced HRV",
    journal = "Nephrol Dial Transplant",
    year    = "2008",
    volume  = "23",
    pages   = "444-449"
}


@Article{reiss2009,
AUTHOR = {Reiss, Philip T and Ogden, R Todd},
TITLE = {Smoothing parameter selection for a class of semiparametric linear models},
JOURNAL = {Journal of the Royal Statistical Society, B},
YEAR = {2009},
VOLUME = {71},
PAGES = {505-523}
}


@Article{reiss2010,
AUTHOR = {Reiss, Philip T and Ogden, R Todd},
TITLE = {Functional generalized linear models with images as predictors},
JOURNAL = {Biometrics},
YEAR = {2010},
VOLUME = {66},
NUMBER = {1},
PAGES = {61-69}
}



@article{rice1991,
    author  = "Rice, J. A. and Silverman, B. W.",
    title   = "Estimating the mean and covariance structure nonparametrically when the data are curves",
    journal = "Journal of the Royal Statistical Society, Series B",
    year    = "1991",
    volume  = "53",
    pages   = "233-243"
}

@ARTICLE{rice2001,
    author = {John A. Rice and Colin O. Wu},
    title = {Nonparametric Mixed Effects Models for Unequally Sampled Noisy Curves},
    journal = {Biometrics},
    year = {2001},
    volume = {57},
    pages = {253--259}
}


@article{robinson1991,
    author = {Robinson, G. K.},
    citeulike-article-id = {756581},
    journal = {Statistical Science},
    keywords = {random-effects, review, statistics},
    number = {1},
    pages = {15--32},
    posted-at = {2006-07-13 10:32:48},
    priority = {0},
    title = {{That BLUP is a good thing: the estimation of random effects}},
    url = {http://www.jstor.org/stable/2245695},
    volume = {6},
    year = {1991}
}


@article{rosen2007,
    author  = "Rosen, O. and Stoffer, D.",
    title   = "Automatic estimation of multivariate spectra via smoothing splines",
    journal = "Biometrika",
    year    = "2007",
    volume  = "94",
    pages  = "335-345",
}

@article{rosen2008,
    author  = "Rosen, O. and Stoffer, D. and Wood, S.",
    title   = "Local spectral analysis via a bayesian mixture of smoothing splines",
    journal = "Journal of the American Statistical Association",
    year    = "2008",
    volume  = "In Press",
}


@article{rosen2012,
    author  = "Rosen, O. and Wood, S. and Stoffer, D.",
    title   = "AdaptSPEC: Adaptive spectral estimation for nonstationary time series",
    journal = "Journal of the American Statistical Association",
    year    = "2012",
    volume  = "107",
    pages  = "1575-1589",
}

@article{ress1995,
    author  = "Ress, K. and Spence, D.P. and Earis, J.E. and Calverley, P.M.",
    title   = "A arousal response from apneic events during non rapid-eye-movement sleep",
    journal = "Am J Respir Crit Care Med",
    year    = "1995",
    volume  = "152",
    page =  "1016-1021"
}

@article{ruppert2002,
    author  = "Ruppert, David",
    title   = "Selecting the number of knots for peanlized splines",
    journal = "Journal of Computational and Graphical Statistics",
    year    = "2002",
    volume  = "11",
    pages   = "735-757"
}

@book{ruppert2003,
    author  = "Ruppert, David and Wand, M. P. and Carroll, R. J.",
    title   = "Semiparametric Regression",
    publisher = "Cambridge Press: New York",
    year    = "2003"
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% s

@article{saavedra2000,
    author  = "Saavedra, P. and Hernandez, C. N. and Artiles, J.",
    title   = "Spectral analysis with replicated time series",
    journal = "Communications in Statistics - Theory and Methods",
    year    = "2000",
    volume  = "29",
    pages   = "2343-2362"
}

@article{saavedra2008,
    author  = "Saavedra, P. and Hernandez, C. N. and Luengo, I. and Artiles, J. and Santana, A.",
    title   = "Estimation of population spectrum for linear processes with random coefficients",
    journal = "Computational Statistics",
    year    = "2008",
    volume  = "23",
    pages   = "79-98"
}


@article{sakiyama2003,
    author  = "Sakiyama, K. and Taniguch, M.",
    title   = "Discriminant analysis for locally stationary processes",
    journal = "Journal of Multivariate Analysis",
    year    = "2004",
    volume  = "90",
    pages   = "282-300"
}

@article{sanderson2010,
    author  = "Sanderson, J. and Fryzlewicz, P. and Jones, M. W.",
    title   = "Estimating linear dependence between nonstationary time series using the locally stationary wavelet model",
    journal = "Biometrika",
    year    = "2010",
    volume  = "97",
    pages   = "435-446"
}

@article{schwarz2016,
    author  = "Katsiaryna Schwarz and Tatyana Krivobokova",
    title   = "A unified framework for spline estimators",
    journal = "Biometrika",
    year    = "2016",
    volume  = "103",
    pages   = "121-131"
}

@article{shumway2003,
    author  = "Shumway, R. H.",
    title   = "Time-frequency clustering and discriminant analysis",
    journal = "Statistics and Probability Letters",
    year    = "2003",
    volume  = "63",
    pages   = "307-314"
}

@book{shumway2011,
    author  = "Shumway, R.H. and Stoffer, D.",
    title   = "Time Series Analysis and Its Applications",
    publisher = "Springer: New York",
    year    = "2011"
}

@book{smith1997,
    author  = "Smith, S.",
    title   = "The Scientist and Engineer's Guide to Signal Processing",
    publisher = "California Technical Publishing: San Diego",
    year    = "1997"
}


@article{staniswalis1998,
    author  = "Staniswalis, J. G. and Lee, J. J",
    title   = "Nonparametric regression analysis of longitudinal data",
    journal = "Journal of the American Statistical Association",
    year    = "1998",
    volume  = "93",
    pages   = "1403-1418"
}

@article{solow2006,
	author  = "Solow, A.",
	title   = "An {ENSO} shift revisited",
	journal = "Geophysical Research Letters",
	year    = "2006",
	volume  = "33",
	pages   = "L22602"
}



@article{sugi2009,
	author  = "Sugi, T. and Kawana, F. and Nakamura, M.",
	title   = "Automatic EEG arousal detection for sleep apnea syndrome",
	journal = "Biomedical Signal Processing and Control",
	year    = "2009",
	volume  = "4",
	pages   = "329-337"
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% t


@book{tapia1978,
    author  = "Tapia, R. A. and Thompson, J. R.",
    title   = "Nonparametric Probability Density Estimation",
    publisher = "Baltimore: Johns Hopkins University Press",
    year    = "1978"
}


@article{thompson1982,
    author  = "Thompson, D. J. ",
    title   = "Spectrum estimation and harmonic analysis",
    journal = "Proceedings of the IEEE",
    year    = "1982",
    volume  = "70",
    pages   = "1055-1096"
}


@article{thompson2008,
    author  = "Thompson, W. K. and Rosen, O. ",
    title   = "A Bayesian model for sparse functional data",
    journal = "Biometics",
    year    = "2008",
    volume  = "64",
    pages   = "54-63"
}



@article{tiao1989,
    author  = "Tiao, G. and Tsay, R.",
    title   = "Model specification in multivariate time series",
    journal = "Journal of the Royal Statistical Society, B.",
    year    = "1989",
    volume  = "51",
    pages   = "157-213"
}

@article{tsay1985,
    author  = "Tsay, R. and Tiao, G.",
    title   = "Use of canonical analysis in time series identification",
    journal = "Biometrika",
    year    = "1985",
    volume  = "72",
    pages   = "299-315"
}

@article{trenberth1996,
	author  = "Trenberth, K. and Hoar, T.",
	title   = "The 1990-1995 {E}l {N}i\~no southern oscillation event: longest on record",
	journal = "Geophysical Research Letters",
	year    = "1996",
	volume  = "23",
	pages   = "57-60"
}

@article{trenberth1997,
	author  = "Trenberth, K. and Hoar, T.",
	title   = "{E}l {N}i\~no and climate change",
	journal = "Geophysical Research Letters",
	year    = "1997",
	volume  = "24",
	pages   = "3057-3060"
}

@article{timmermann2004,
	author  = "Timmermann, A. and Jin, F. and Collins, M.",
	title   = "Intensification of the annual cycle in the tropical {P}acific due to greenhouse warming",
	journal = "Geophysical Research Letters",
	year    = "2004",
	volume  = "31",
	pages   = "L12208"
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% v

@article{vanoli1996,
    author  = "Vanoli, E. and Adamson, P.B. and Ba-Lin, Pinna G.D., and Lazzara, R. and Orr, W.C.",
    title   = "Heart rate variability during specific sleep stages. A comparison of healthy subjects with patients after myocardial infarction",
    journal = "Circulation",
    year    = "1996",
    volume  = "91",
    pages   = "1918-1922."
}



@book{verbeke2000,
    author  = "Verbeke, Geert and Molenberghs, Geert",
    title   = "Linear Mixed Models for Longitudinal Data",
    publisher = "New York: Springer",
    year    = "2000"
}

@article{vonsachs1994,
    author  = "von Sachs, R.",
    title   = "Peak-insensitive non-parametric spectrum estimation",
    journal = "Journal of Time Series Analysis",
    year    = "1994",
    volume  = "15",
    pages   = "429-452"
}

@article{vecchi2010,
	author  = "Vecchi, G. and Wittenberg, A.",
	title   = "{E}l {N}i\~no and our future climate: where do we stand?",
	journal = "Wiley Interdisciplinary Reviews: Climate Change",
	year    = "2010",
	volume  = "1",
	pages   = "260-270"
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% w

@Article{wahba1980,
  author="Wahba, G.",
  title="Automatic smoothing of the log-periodogram",
  journal="Journal of the American Statistical Association",
  volume=75,
  year=1980,
  pages="122-132"
}

@Article{wahba1983,
  author="Wahba, Grace",
  title={{B}ayesian ``confidence intervals'' for the cross-validated smoothing spline},
  journal="Journal of the Royal Statistical Society, Series B",
  volume=45,
  year=1983,
  pages="133-150"
}

@Article{wahba1985,
  author="Wahba, Grace",
  title={A comparison of {GCV} and {GML} for choosing the smoothing parameter in the generalized spline smoothing problem},
  journal="Annals of Statistics",
  volume=13,
  year=1985,
  pages="1378-1402"
}

@book{wahba1990,
    author  = "Wahba, G.",
    title   = "Spline Models for Observational Data",
    publisher = "(CBMS-NSF Regional Conference Series in Applied Mathematics), Philadelphia: SIAM",
    year    = "1990"
}


@Article{wang1995,
  author="Wang, Yuedong and Wahba, Grace",
  title={Bootstrap confidence intervals for smoothing splines and their comparison to {B}ayesian ``confidence intervals''},
  journal="Journal of Statistical Computation and Simulation",
  volume=51,
  year=1995,
  pages="263-279"
}

@Article{wang1998jasa,
  author="Wang, Y.",
  title="Smoothing spline models with correlated random errors",
  journal="Journal of the American Statistical Association",
  volume=60,
  year=1998,
  pages="159-174"
}

@Article{wang1998jrssb,
  author="Wang, Y.",
  title="Mixed-effects smoothing spline ANOVA",
  journal="Journal of the Royal Statistical Society B",
  volume=60,
  year=1998,
  pages="159-174"
}

@Article{wang1998comment,
  author={Wang, Y. and Wahba, G."},
  title={Discussion of `Smoothing Spline Models for the Analysis of Nested and Crossed Samples of Curves' by Brumback and Rice},
  journal={Journal of the American Statistical Association},
  volume={93},
  year={1998},
  pages={976-980}
}




@book{wang2011,
    author  = "Wang, Y.",
    title   = "Smoothing Splines: Methods and Application",
    publisher = "London: Chapman \& Hall/CRC",
    year    = "2011"
}

@article{wand2008,
    author = "Wand,  M. P. and Ormerod,  J. T.",
    journal = {Australian and New Zealand Journal of Statistics},
    month = {June},
    number = {2},
    pages = {179--198},
    posted-at = {2008-07-15 14:26:02},
    publisher = {Blackwell Publishing},
    title = {On semiparametric regression with O'Sullivan penalized splines},
    url = {http://dx.doi.org/10.1111/j.1467-842X.2008.00507.x},
    volume = {50},
    year = {2008}
}


@Article{wang2003,
  author="Wang, N.",
  title="Marginal nonparametric kernel regression accounting for within-subject
correlation",
  journal=bio,
  volume=90,
  year=2003,
  pages="43-52"
}


@Article{whittle1953,
  author="Whittle, P.",
  title="Estimation and information in stationary time series",
  journal="Arkiv f{\"o}r Matematik",
  volume=2,
  year=1953,
  pages="423-434"
}


@incollection{whittle1954,
  author="Whittle, P.",
  title="Some recent contributions to the theory of stationary processes",
  booktitle="A Study in the Analysis of Stationary Time Series",
  edition=2,
  year=1954,
  pages="196-228",
  editor="Wold, H.",
  publisher="Almqvist and Wiksell",
  address="Uppsala"
}


@article{welsh2002,
    author  = "Welsh, A. and Lin, X., and Carroll, R. J.",
    title   = "Marginal longitudinal nonparametric regression: locality and efficiency of spline and kernel methods",
    journal = "Journal of the American Statistical Society",
    year    = "2002",
    volume  = "97",
    pages   = "482-493"
}



@ARTICLE{wood2011,
title = {Fast stable restricted maximum likelihood and marginal likelihood estimation of semiparametric generalized linear models},
author = {Wood, S. N.},
year = {2011},
journal = {Journal of the Royal Statistical Society, B},
volume = {73},
pages = {3-36}
}

@ARTICLE{wu2002,
title = {Local Polynomial Mixed-Effects Models for Longitudinal Data},
author = {Wu, H. and  Zhang, J-T.},
year = {2002},
journal = {Journal of the American Statistical Association},
volume = {97},
pages = {883-897}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% y

@article{yang2016,
    author  = "Yang, Wen-Hsi and Holan, Scott H. and Wikle, Christopher K.",
    title   = "Bayesian lattice filters for time-varying autoregression and time-frequency analysis",
    journal = "Bayesian Analysis",
    year    = "2016",
    pages   = "In Press."
}


@article{yao2005,
    author  = "Yao, F. and Muller, H.-G. and Wang, J.-L.",
    title   = "Functional Data Analysis for Sparse Longitudinal Data",
    journal = "Journal of the American Statistical Society",
    year    = "2005",
    volume  = "100",
    pages   = "577-590"
}

@article{yao2006,
    author  = "Yao, F. and Lee, T. C. M",
    title   = "Penalized spline models for functional principal components analysis",
    journal = "Journal of the Royal Statistical Society, Series B",
    year    = "2006",
    volume  = "68",
    pages   = "3-25"
}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% z


@article{zhang2007,
    author  = "Zhang, J.-T. and Chen, J.",
    title   = "Statistical inferences for functional data",
    journal = "Annals of Statistics",
    year    = "2007",
    volume  = "35",
    pages   = "1052-1079"
}


@article{zaremba1968,
    author  = "Zaremba, S. K.",
    title   = "Some applications of multidimensional integration by parts",
    journal = "Annales Polonici Mathematici",
    year    = "1968",
    volume  = "21",
    pages   = "85-96"
}

@book{zygmund2003,
    author  = "Zygmund, A.",
    title   = "Trigonometric Series",
    publisher = "Cambridge: Cambridge University Press",
    year    = "2003"
}

@article{zhang2016,
	author={Zhang,Shibin},
	year={2016},
	title={Adaptive spectral estimation for nonstationary multivariate time series},
	journal={Computational Statistics \& Data Analysis},
	volume={103},
	pages={330-349}


%%%%%%%%%%%%
@article{arousal1992,
	author ={ASDA},
	year={1992},
	title={{EEG} arousals: scoring rules and examples: a preliminary report from the {S}leep {D}isorders {A}tlas {T}ask {F}orce of the {A}merican {S}leep {D}isorders {A}ssociation},
	journal={Sleep},	
	volume={15},
	pages={173}
}

